Towards Higher Order Oscillatory Ising Machines

Ising machines as hardware solvers of combinatorial optimization problems (COPs) can efficiently explore large solution spaces due to their inherent parallelism and physics-based dynamics. Many important COP classes such as satisfiability (SAT) assume arbitrary interactions between problem variables, while most Ising machines only support pairwise (second-order) interactions. This necessitates translation of higher-order interactions to pair-wise, which typically results in extra variables not corresponding to problem variables, and a larger problem for the Ising machine to solve than the original problem. This in turn can significantly increase time-to-solution and/or degrade solution accuracy. In this paper, considering a representative CMOS-compatible class of Ising machines, we propose a practical design to enable direct hardware support for higher order interactions. By minimizing the overhead of problem translation and mapping, our design leads to up to 4x lower time-to-solution without compromising solution accuracy.

==> Sections/Motivation.tex <==
% \redHL{make the case for SAT, that it is the original NP-complete problem, representative, others can be translated to SAT etc. ...}
%SAT (Boolean satisfiability) is a foundational problem in computer science, known to be NP-complete~\cite{cormen2022introduction}. It was the first problem proven to be NP-complete, serving as the starting point for the theory of NP-completeness. Any other NP-complete problem can be transformed into SAT using a polynomial-time reduction~\cite{karp2010reducibility}.
%SAT problems are excellent examples of higher-order interactions because they involve logical expressions that can require simultaneous relationships between multiple variables. Specifically, SAT problems ask whether there exists an assignment of truth values (true or false) to variables that satisfies a given Boolean formula, which is often represented in Conjunctive Normal Form (CNF). Each clause in the CNF formula typically involves logical OR operations over several variables or their negations, representing higher-order interactions.


% \redHL{before we can explain this figure, we need to provide more detail/insight on how variables get mapped to spins.} 
We will start our discussion with an illustrative example using SAT as a representative COP featuring higher-order interactions between problem variables. 
%\blueHL
{
%{To map SAT problem variables to Ising spins (or equivalently, QUBO variables), 
For problem translation, we first establish a correspondence between Boolean variables in the SAT formulation and binary or spin variables in QUBO or Ising models. 
%In a n-variable, m-clause SAT instance, the mapping begins by associating each of the n SAT variables with one QUBO or Ising spin, maintaining a one-to-one correspondence. 
%However, SAT clauses induce logical constraints 
%that require additional structure in the optimization model. To represent these constraints 
Each SAT clause induces a constraint,
which should be expressed
within the pairwise interaction limits of QUBO or Ising formulations
%logical constraints of each clause 
as a {\em quadratic} objective function over binary variables (which boils down to a clause specific Hamiltonian, with the order of interactions being limited to at most two), and
%with 
%, where 
satisfying assignments must minimize this objective function, by construction.
%correspond to low-energy states. 
This is when ancillary 
%(auxiliary) 
variables are introduced. 

%For example, 
Considering the generic 3-SAT clause  \( (x_1 \lor x_2 \lor x_3) \), translating the cubic interaction among the problem variables \( x_1, x_2 \text{, and } x_3 \) %, once converted 
into the equivalent quadratic expression 
(i.e., {\em quadratization}),
%if we want to model its satisfaction condition directly in an energy function. Due to the pairwise interaction limit of the Ising model, we 
%need to reduce or ``quadratize'' them -- i.e., convert them into equivalent quadratic expressions. This process 
%necessitates 
typically results in new binary variables (ancillaries) to express the cubic interaction 
%that mediate the interaction, enforcing the higher-order relationship 
through extra 
terms which penalize unsatisfying assignments~\cite{cilasun2024sat}.
%by formulating variable-to-variable interactions. 
How such extra terms look like and how many ancillary variables each necessitate to encode problem-specific correlations among problem variables depend on the mathematical formulation.  
%penalty terms. %If the problem contains many such clauses, it 
A typical problem contains many such clauses 
%and inherently represents a system 
with possibly overlapping higher-order interactions, which complicates 
mathematical formulation
%problem translation 
further.

To translate an $n$-variable $m$-clause 3-SAT instance, even the highly compact formulation proposed by Chancellor~\cite{Chancellor2016} introduces an ancillary variable for each clause, resulting in a total of $n$+$m$ variables in the translated problem. Alternatively, in the Integer Linear Programming (ILP)-based formulation proposed by~\cite{cilasun2024sat}, the encoding uses two ancillary variables per clause to model clause Hamiltonians as equality constraints, yielding a total of $n$+2$m$ variables in the translated problem. These additional variables ensure that multi-variable logical expressions are correctly transformed into pairwise (quadratic) energy penalties, making the SAT-to-Ising (or equivalently QUBO) mapping both physically implementable and mathematically correct. In contrast to these formulations, mapping a SAT instance to HOIMs requires to solve a Polynomial Unconstrained Binary Optimization (PUBO)~\cite{nagies2025boostingquantumannealingperformance} problem instead of QUBO -- which we %define as 
will generally refer to as 
Higher-order Unconstrained Binary Optimization (HUBO) thoughout the paper}, and which eliminates the need for ancillary variables by definition. 
%Thus, beyond pairwise relationships can be mapped without using any ancillary variables.

Figure \ref{fig:spincount} shows  
%(equivalently QUBO) 
spin count in the translated problem as a function of problem size, using different formulations for mapping higher-order SAT interactions. \blueHL{The details of the mapping have been covered in detail in Section~\ref{sec:Implementation}.}
%to pair-wise Ising (QUBO) interactions. 
The x-axis covers 3-SAT problems from SATLIB ~\cite{SATLIB} of increasing problem size -- 20, 50, 100, and 200 variables.
%spin counts for SATLIB benchmarks~\cite{SATLIB} with 20, 50, 100, and 200 variables after mapping to 
We consider QUBO (Chancellor, ILP) and HUBO formulations.
%\footnote{}
%using the Chancellor, ILP, and HUBO formulations, respectively.
%assuming all-to-all connectivity without loss of generality. 
% \redHL{what are these formulations? Can be addressed in the previous paragraph or here; need references. We also need to explain what these benchmarks are, where they are coming from, why representative etc. What is spin count? Is this Ising or QUBO mapping? etc. Also, what is ``Quartic''? Is this is the hypothetical best case or HOIM?}
%\blueHL
{The plot clearly shows that as the problem size increases from 20 to 200 variables, the HUBO formulation significantly reduces the overall spin count by eliminating the need for ancillary spins. 
%to represent them. 
%In all cases, the HUBO formulation yields a significant reduction in spin count, 
Specifically, HUBO requires $\approx 5.5\times$ fewer spins than the most efficient QUBO formulation \textit{Chancellor} for 20 variable problems and $\approx 5.3\times$ for 200 variable problems, highlighting its scalability and encoding efficiency for larger SAT instances.} 
% \redHL{add some numbers from the fig. here on dramatic reduction; i.e., compare best performing pairwise formulation to quartic for each problem size and report the reduction factor in spin count}



% \redHL{brief explanation of CNF to Ising mapping would help here, if possible. a high level insight on why extra variables are needed. if we need math to do so we can expand this in the background section. we also need to cover what k in k-SAT is, which ks are common etc.}

%\blueHL{To map a CNF formula to an equivalent Ising model, the Boolean logic is first transformed into a Quadratic Unconstrained Binary Optimization (QUBO) problem. This formulation encodes the logical constraints of each clause as a quadratic objective function over binary variables, where satisfying assignments correspond to low-energy states. However, since the Ising model natively supports only linear and pairwise (quadratic) interactions, ancillary variables are introduced to decompose higher-order logical terms into quadratic/pairwise components. This becomes particularly relevant in k-SAT problems, where each clause contains up to k literals. Among these, 3-SAT (k = 3) is most commonly studied, as any k-SAT instance with k $>$ 3 can be efficiently reduced to an equivalent 3-SAT form in polynomial time.}

%These higher-order dependencies in SAT problems make them ideal for demonstrating the need for computational models, such as Higher-Order Ising Machines (HOIMs), that can natively handle interactions beyond pairwise. HOIMs can directly encode the logic of multi-variable interactions in SAT problems, avoiding the need for transformations like quadratization. Consequently, SAT problems serve as a compelling use case for exploring the advantages of solving higher-order interactions in optimization frameworks.

\begin{figure} [htp]
    \centering
    %\includegraphics[width=0.9\linewidth]{Figures/spin-count.png}
    \includegraphics[width=0.85\columnwidth]{Figures/spin-count.png}
    \caption{
    Ising spin (equivalently, QUBO variable) count in the translated problem as a function of problem size, using different formulations for mapping higher-order SAT interactions.
%to pair-wise Ising (QUBO) interactions. 
x-axis covers 3-SAT problems from SATLIB ~\cite{SATLIB} of increasing problem size.}
    %Ising spin count in the translated problem as a function of problem size, using different formulations for translating higher-order SAT interactions to pair-wise Ising interactions. x-axis covers 3-SAT problems of increasing problem size. 
    % \redHL{Ilp uppercase; y-axis: Spin Count}
    \label{fig:spincount}
    %\vspace{-.5cm}
\end{figure}
